Beyond Duplicates: Towards Understanding and Predicting Link Types in Issue Tracking Systems

Software projects use Issue Tracking Systems (ITS) like JIRA to track issues and organize the workflows around them. Issues are often inter-connected via different links such as the default JIRA link types Duplicate, Relate, Block, or Subtask. While previous research has mostly focused on analyzing and predicting duplication links, this work aims at understanding the various other link types, their prevalence, and characteristics towards a more reliable link type prediction. For this, we studied 607,208 links connecting 698,790 issues in 15 public JIRA repositories. Besides the default types, the custom types Depend, Incorporate, Split, and Cause were also common. We manually grouped all 75 link types used in the repositories into five general categories: General Relation, Duplication, Composition, Temporal / Causal, and Workflow. Comparing the structures of the corresponding graphs, we observed several trends. For instance, Duplication links tend to represent simpler issue graphs often with two components and Composition links present the highest amount of hierarchical tree structures (97.7%). Surprisingly, General Relation links have a significantly higher transitivity score than Duplication and Temporal / Causal links. Motivated by the differences between the link types and by their popularity, we evaluated the robustness of two state-of-the-art duplicate detection approaches from the literature on the JIRA dataset. We found that current deep-learning approaches confuse between Duplication and other links in almost all repositories. On average, the classification accuracy dropped by 6% for one approach and 12% for the other. Extending the training sets with other link types seems to partly solve this issue. We discuss our findings and their implications for research and practice.

==> figures/DCCNN_performance.tex <==
\begin{figure*}
    \centering
         \centering
        \includegraphics[width=0.85\textwidth]{Pictures/DCCNN_all.png}
       \caption{DCCNN model. Macro F1, Accuracy, and ROC-AUC Score for projects and dataset combinations. The projects are ordered by amount of links.}
\label{fig:DCCNNPerformance}
\end{figure*}

==> figures/SCCNN_performance.tex <==
\begin{figure*}
    \centering
         \centering
        \includegraphics[width=0.85\textwidth]{Pictures/SCCNN_all.png}
       \caption{SCCNN model. Macro F1, Accuracy, and ROC-AUC score for projects and dataset combinations. The projects are ordered by amount of links.}
\label{fig:SCCNNPerformance}
\end{figure*}

==> figures/link_usage.tex <==
\begin{figure}
     \centering
         \centering
         \includegraphics[width=0.3\textwidth]{Pictures/link_cat_usage_cleaned.png}
         \vspace{-0.5cm}
         \caption{Usage of link categories across studied repos (in \%).}\label{fig:LinkUsage}
    %   \vspace{-0.5cm}
\end{figure}

==> figures/model_performance.tex <==
\begin{figure*}
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.95\textwidth}
    \centering
    \includegraphics[scale=0.5]{Pictures/SCCNN_f1.png}
    \caption{Macro F1-scores of the different categories across the ITS for SCCNN}
    \label{fig:SCCNNF1}
\end{subfigure}
\begin{subfigure}[b]{0.95\textwidth}
    \centering
    \includegraphics[scale=0.5]{Pictures/DCCNN_f1.png}
    \caption{Macro F1-scores of the different categories across the ITS for DCCNN}
    \label{fig:DCCNNF1}
\end{subfigure}
\caption{Performance of the SCCNN and DCCNN models on the JIRA ITS.}
\label{fig:model_performance}
\end{figure*}

==> oldmain.tex <==
\begin{abstract}
%------SHORTEN?------
Issue tracking systems are powerful tools that can help increase the efficiency of software development activities. 
% Bug reports are important indicators of requirements defects, that are overlooked during the development stage.
However, these tools may miss their purpose when their issue reports are ill-documented and inter-dependencies are missing or unclear. 
% However, ill-documented bug reports with missing or unclear inter-dependencies make the task of tracing bug reports to requirements a tedious one.
% Particularly in large issue tracking system, stakeholders are faced with information overload.
When it comes to issue inter-dependencies, duplicate issue detection has been the focus of research. Little effort has been done to automatically detect and document other issue dependency types, which are predominately project-specific.
% In this work, we present a new approach for link discovery between bug reports in issue tracking systems.
% Contrary to the common approach of comparing two issues and evaluating their similarity, as is done in duplicate-dependency research, we compare two links, each consisting of two issues, and evaluate their similarity. 
We propose to fill this research gap by implementing a new approach by checking for similarity of two issue inter-dependencies, whereby an inter-dependencies is an embedded representation of two issues
% Contrary to the common approach of comparing two bug reports and evaluating whether they have a certain link type e.g. duplicate, we encode the (links) between the bug reports and compare these, which allows us to generalise to all link types.  
If they are the same inter-dependency type they should be similar and if they are different inter-dependency types that are defined with enough examples in an issue tracking system.
For this, we use a Siamese neural network architecture to find the similarity between two inter-dependencies.
As this model is more complex, we need more training data, however since we view inter-dependencies as the input, we automatically boost the amount of available training data.
At the same time, we reduce the dimension/size of the output, by converting from a multi-class approach to a binary approach. 
We evaluated this approach on the data contained in Apache's and Qt's issue tracking system, Jira.
When replicating the siamese network approach from Deshmukh et al.~\citep{DESHMUKH17} to the Apache and Qt data, we achieved an
%% UPDATE RESULTS
accuracy of 70\%, once we adapted this approach to all inter-dependency types found in Qt's Jira, the accuracy dropped to 35\%, with our approach we achieved an accuracy of 60\%.

%Story:
%customisable model to be tailored to own data
%more link types than normal (duplicates)

% This work tries a new approach at the problem of finding links between issues in issue tracking systems (ITS).
% Instead of comparing two issues and evaluating if these issues have a link, e.g. are duplicates of each other, we compare two links and evaluate whether they are the same link, this is then generally applicable to all link types (such as duplicate, dependency, no relation, related, parent-child)
% For this we first encode the issues (title, description, properties) and then use the output of two issues to model the link between them by feeding this into an additional network. This link encoding is then used as input in a Siamese network to find the similarity of two links (each a pair of issues). This boosts the amount of training data.

Keywords: Dependencies/Links in ITS, duplicate detection of bug reports, Recommender systems, similarity detection, link detection between artifacts

\end{abstract}

\maketitle

% Structure:
% - Introduction
% - Research Settings
% -- RQs
% -- Data (Acquisition, Label, Prep) 
% - Experiment Setup
% -- NN Architecture
% -- Hyperparameters
% -- Evalutation
% - Experiment Results
% - Related Work
% - Discussion 
% -- Implication
% -- Threats to Validity
% - Conclusion & Future Work

\section{Introduction}\label{sec:Introduction}
% - Problem case
% - Current benchmarks
% - new dataset
% - multiple links

%- ITS as a basis for software engineering.
% Issue tracking systems are an important tool in organization to organize issues that need to be taken care of. In Software Engineering it is a basis for a good software product.
Issue tracking systems (ITS) have become an important component of the software development tool landscape. Crucial tasks such as release management are hardly imaginable nowadays without the assistance of an issue tracker.
% Issue reports usually consist oft many different information. 
Independently of the issue tracker used, an issue report commonly consists of text fields, such as a title, a description and comments from stakeholder and property fields, such as the status, the resolution, the affected version, the type and also different inter-dependencies to other issues.
% - Issues are connected to each other, they can be duplicates or requires relationships between them, we will refer to the different type of relationships as \textit{links}.
In this work, our focus lies on identifying unknown or missing inter-dependencies between issues, these inter-dependencies can have different types, common are \textit{duplicates}, \textit{requires} and \textit{relates} inter-dependency types.
Manually finding and marking these inter-dependencies grows quadratic with the size of the issues in the issue tracking system, at one point this is impossible for humans to organize and sort. 
Additionally, adding more inter-dependencies to a system can be harder than needed depending on the UI and usability.
%(Cite paper on information overload and problems with ITS)
There has already been a great amount of work into identifying duplicates in issue tracking system. Deshmukh et al.~\citep{DESHMUKH17} tested a siamese network approach with the duplicate data set of NetBeans, Eclipse and Open office with a accuracy of 0.822 while Xie et al.~\citep{XIE18} used Convolutional Neural Networks to identify duplicates in bug reports from Hadoop, Spark, HDFS and Mapreduce with an accuracy of 0.941 and an F1-score of 0.930.
%- A lot of research on finding duplicates (name data sets and benchmarks with papers)
We tackle this problem on another data set which provides a variety of inter-dependencies, namely the issues from Qt's Jira. 
This data set contains 6 different inter-dependency types, \textit{duplicates}, \textit{requires}, \textit{replaces}, \textit{work breakdown}, \textit{relates} and \textit{tests}.
First, we used the approach from previous research to identify only \textit{duplicates} to get a baseline for this data set. Second, we generalized this model to predict all different kinds of inter-dependencies by adjusting the output layer. Third, we created a more complex model where we view the problem from another angle that increases amount of training data while reducing the output to a binary classification from a multi-class classification to achieve better results. 
% This is done by computing the similarity between links instead of issues.

% Debugging in software engineering is mainly focused on establishing the relationship between bug reports and software artifacts. 
% However, software bugs may have a different origin than the source code itself.
% In fact, requirement defects are one very costly source of software failures [find citation on cost of maintenance].
% Therefore, it is necessary to establish the link between requirements defects and bug reports to prevent future occurrences of the same defect.
% Requirements are often organised into documents, where the dependencies between single requirements are maintained.
% Bug reports, on the other hand, are often documented as separate issues within issue tracking systems and their dependencies often remain undocumented to the exception of the duplicate relationships rendering a bug report almost redundant. Other types of links might include "Relat
% This is likely due to the fact that link discovery between bug reports is a tedious manual task, which exponentially grows in complexity with the number of bug reports as the potential link between each two bug reports needs to be considered.

% To counter this problem, we present a new deep learning approach of bug report link discovery.
% The novelty of the approach lays not only in the architecture but also in its capability to accept different bug report structures independently of the issue tracking system.
% We test our approach on two open source issue tracking repositories namely Qt using the JIRA issue tracking system and Eclipse using the Bugzilla issue tracking system.

% should be re-formulated
This paper is organised as follows: in section~\ref{sec:research_settings} we discuss the research questions and the data used in this work, in section~\ref{sec:experiment_setup} we discuss the architecture of the neural networks and how we evaluated their performance, in section~\ref{sec:experiment_results} we present the results of our research, in section~\ref{sec:related_work} we discuss other approaches that tackled a similar problem, in section~\ref{sec:discussion} we discuss the implications and threats to validity and finally, in section~\ref{sec:conclusion} we conclude this work and present future possibilities. 

\section{Research Settings}\label{sec:research_settings}
% - RQs
% - Data (Acquisition, Label, Prep) 
In this section we introduce our research questions and present the data we used for this work.

\subsection{Research Questions}

%should this be moved to the introduction?

\textbf{RQ1.} How well does Deshkmuk et al approach / other duplication detection strategies work on Qt's issue data?\\
\textbf{RQ2.} Can these approaches be generalized to different inter-dependency types and not only duplication?\\
\textbf{RQ3.} By "duplicating" the network can we improve the inter-dependency detection for multiple types? How does it compare to the simpler approach?\\

\subsection{Data set}
In the following we describe our data collection and pre-processing process.
Issue tracking systems contain sensitive information and are not usually made public by software companies.
We therefore turned to an large open source issue tracking system as a data source, namely Qt’s Jira \footnote{\url{https://bugreports.qt.io/}}. This Jira consists of different projects for the different parts of the Qt framework, the largest is \textit{QTBUG} with 72,009 issues followed by \textit{QTCREATORBUG} with 20,725 issues. All other projects have less than 3,000 issues. In total there are 19 projects. We extracted the title, description and the inter-dependency from Qt's Jira data.
Additionally, this issue tracking system contains a diverse amount of inter-dependency types besides \textit{duplicates}. The distribution of the different inter-dependency types between two issuez is shown in figure~\ref{fig:linktype_distribution}.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Pictures/linktypes_dist.png}
    \caption{Distribution of inter-dependencies of issues in Qt's Jira}
    \label{fig:linktype_distribution}
\end{figure}
%- has multiple links (statistic of link distribution), inside one project and cross-project

These inter-dependencies are defined either within the same project or across projects. 
In this data set 13,783 (90,8\%) are inter-project inter-dependencies and 1,393 (9,2\%) are cross-project. 

To collect the bug reports, we scraped both issue tracking systems using a customized python script in early 2019.
This resulted in a data set of 108,074 issues, of which 19958 have at least on inter-dependency.
The average number of inter-dependencies per issue is 0.28, which is fairly low. 

% \begin{table}[!h]
%   \caption{Overview of the bug report dataset}
%   \label{tab: dataset}
%   \begin{tabular}{lrr}
%     \toprule 
%      &  Eclipse Bugzilla & Qt Jira\\
%     \midrule
%     \# Issues   &   532,595  & 108,074 \\
%     \# Issues with links   &  &\\
%     \# Link types   &  &\\
%     Average links per issue   &  &\\
%   \bottomrule
% \end{tabular}
% \end{table}
We added a \textit{No inter-dependency} type to our data set, as a classifier also needs examples for no inter-dependencies to generate good results. 
As some issues have the resolution "Duplicate", but no \textit{duplicates} inter-dependency, we deleted issues with that resolution from the pool of issues from which we created the \textit{No inter-dependency} examples. Of course, it is possible that we create a "No inter-dependency" between two issues that have an inter-dependency, but with our heuristic we lowered the chance of this happening.
We added about 5,000 of this \textit{No inter-dependency} type, as this is similar in size to the biggest class.
%Additionally, we generated them in a way to mirror the distribution of inter-dependencies of the projects.
We also disregarded \textit{tests} as a class, as there are only 12 instances of this inter-dependency types.
As the data set is imbalanced we used a generator function to randomly pick training examples from a pool where each inter-dependency type has the same probability to be picked.
% Furthermore, in the Jira of Qt the inter-dependencies also have a direction, which we also disregarded as this does not change the inter-dependency type and is not of importance for the classification. 
Despite the Qt issue inter-dependencies having a direction, the latter is not important for the classification and is therefore not further investigated following our approach.
However, future research could also try to identify the direction of the inter-dependency, but this is outside the scope of this paper.
% but this is a harder problem which can be solved after identifying undirected inter-dependencies.
For the more complex network we randomly picked two links from the inter-dependency types, if they are the same type, they received the label "Same Type", if there are from different types, they received the label "Different Type". We ensured that there are the same amount of these two labels to achieve a balanced training set.
The input features for our experiments were the title and description of four issues and their respective inter-dependency types.
The input texts for the neural networks were pre-processed by contractions and symbols not contained in glove embeddings and also putting an empty space between symbols and characters, e.g. turning "(in" to "( in".
Additionally, we checked words during the embedding, e.g. "The" did not receive a word embedding, whereas "the" got one, therefore we also looked at the lower-cased version of a word of the glove word embeddings. 
More complex pre-processing was not done, as lemmatizaing and stemming can negatively impact results according to Camacho-Collados et al.~\citep{CAMACHO_COLLADOS18}. 
Although by lower-casing we risk introducing ambiguity, e.g. Windows, the object instead of the operating system, we manually checked the instances of these ambiguous words which appeared more often. 
Other words that did not have a glove word embedding were part of code fragments or stacktraces and thus not expected to have an embedding.
% Qt Data
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.125]{Pictures/example_Bug_Qt.jpg}
%     \caption{Example Bug report with issue links}
%     \label{fig:example_qt_issue}
% \end{figure}

% \subsubsection{Data Pre-processing}
% Following the example of Deshmukh et al. \cite{DESHMUKH17}, we focus on a reduced set of features derived from the collected bug reports.
% These are the \textit{title}, the \textit{description} and a set of properties including: the \textit{resolution}, the \textit{status} and the \textit{type}, referring to the issue type being bug, task, suggestion, etc. (do we not consider only bugs? - Qts Jira contains a lot of issues, not only bugs, which are related to each other)

\section{Experiment Setup}\label{sec:experiment_setup}
% - Used NN Architectures with pictures
% - Explain layers
% - Hyperparameters
% -- What hyperparameters and which did we choose
% - Evalutation
% -- Metrics used to compare approaches
In this section we describe the different deep learning techniques we used to tackle the problem. We also discuss how we evaluated the different approaches.

\subsection{Neural Network Architecture}
% Explain layers
% Introduce different architectures
% Needs picture
In the experiment we used a mix of RNN, CNN, and dense layers, with a focus on CNN layers as they have proven to work well for text classification tasks~\citep{KIM14, ZHANG15}. RNN are traditionally used for text classification tasks, but take longer to train. CNN was originally used for image classification tasks, but can be also used on text data as it is good in identifying structures inside the input. 
The approach we leaned on was Deshmukh et al.'s~\citep{DESHMUKH17}. 
It uses a siamese network architecture to find duplicates by encoding description and title of an issue. This is then used in a max-margin-objective. 
Issues which are duplicates should be close together and issues which are not duplicates should be far away from each other.
As the issues encoded are their content one could assume to use the encoded issues as input and ask "What type of link do these two issues have?" instead of asking "Are these two issues duplicates?". This is harder to solve as we have a multi-class classification problem and not a binary one which can be elegantly solved by max-margin.
Our idea to improve the mulit-class classification task is to mirror the siamese network and turn this multi-class classification back to a binary classification by asking "Are these two inter-dependencies the same inter-dependency?".
As input for the we used glove word-embeddings for the title and description of the four issues of two inter-dependencies.
On a more concrete level we have some choices to make, we can encode the word-embeddings of the title and description and concatenate the encoded vectors and use this as an issue, which we can encode again and concatenate the encoded issues as a way to represent the links which we can encode again. 
We tried all different 8 combinations for the complex approach, encoding the different parts of a inter-dependency, although each further encoding makes the network more complex:
\begin{itemize}
    \item  No encoding, description and titles are concatenated and fed into a CNN
    \item  Encoding of the description and titles
    \item  Encoding of the issues which are the non-encoded title and description
    \item  Encoding of the links which are the non-encoded titles and description of both issues of the link
    \item  Encoding the issues which are the encoded title and description
    \item  Encoding of the links which are the encoded titles and description of both issues of the link
    \item  Encoding of the link which are the encoded issues without encoding titles and descriptions of the issues
    \item  Encoding all parts, the title and description, issues, and links
\end{itemize}

In Figure~\ref{fig:lynx_network} we show the basic idea of our approach.
The different layers can be skipped and the input can be taken from the previous layer. 
The more layers are chosen, the more complex is the network and thus more prone to overfitting and in the need for more data.
\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{Pictures/LYNXMODEL.png}
    \caption{LYNX network architecture}
    \label{fig:lynx_network}
\end{figure*}

% Another approach could be to first confirm the existing of a link and then determine the type. %Find some research for this approach

\subsection{Hyperparameters}
Choosing the the best performing hyperparameters is harder for deep learning as for traditional methods like SVM or logistic regression~\citep{ZHANG15}. We have to test for the following parameters:
\begin{itemize}
    \item input word vector representation
    \item filter region 
    \item feature maps
    \item activation functions
    \item pooling strategy
    \item regularization terms
    \item batch size
    \item no of periods
    \item learning rate
\end{itemize}
In order to optimize this project we sticked to the advice of Zhang and Wallace in their paper~\citep{ZHANG15}, but had to keep in mind some restrictions in regard to computing time.
In Table~\ref{tab:parameters} we present the different values we chose to test for the different parameters.
\begin{table}[!h]
  \caption{Overview of the parameters configurations explored}
  \label{tab:parameters}
  \begin{tabular}{l | r}
    \toprule 
    parameter & tested values\\
    \midrule
    input word vector representation & static glove \\
    filter region & $\{1,...,10\}$\\
    feature maps & 100, 200, 300, 400, 500, 600\\
    activation functions & relu and tanh \\
    pooling strategy & 1-max pooling\\
    regularization terms & l2\\
    batch size & 32, 64, 128 \\
    no of periods & 10, 25, 50\\
    learning rate & ??\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Evaluation}
We report the accuracy, F1-score, precision and recall (maybe also ROC and AUROC) to evaluate, compare, and interpret the results. 
In case of multi-class we chose to macro-average the scores and give equal weights to the classes. 
Additionally, to compare the results of the complex architecture with the binary output and the simpler architecture with the multi-class output we looked at the performance on the test set.
We used a a 5-fold cross-validation to evaluate the different approaches. This means we trained on 80\% of the data and tested on 20\% of the data and then averaged the results.

\section{Experiment Results}\label{sec:experiment_results}
Adapting the network architecture of Deshmukh et al.~\citep{DESHMUKH17} to a case with multiple inter-dependency types, as we outlined here, is better than just using multiclass with Deshmukh et al.'s architecture. (really need to check this as we cannot simply compare accuracies)

\begin{table*}[]
    \centering
    \begin{tabular}{l|r r r r}
         Approach & Accuracy & F1 & Precision & Recall  \\
         \hline
         Duplicate Replication (Deshmukh et al.) & 0.612 & & & \\
         All Links Replication & 0.359 & & & \\
         Complex Architecture & 0.573 & & &
    \end{tabular}
    \caption{Prelim results}
    \label{tab:my_label}
\end{table*}

\section{Related Work}\label{sec:related_work}
%General
 Wang et al. \citep{WANG08} proposed an approach based on the natural language information contained in bug reports as well as execution information to determine if the bug report is a duplicate of another.
 They calibrated their approach based on the Eclipse bug repository and applied it to the Firefox bug repository resulting in the detection of 67\% to 93\% of duplicate bugs.
 Xie et al. \citep{XIE18} use word embeddings and CNNs to detect duplicate bug reports and evaluate their approach on bug reports taken from JIRA and Bugzilla resulting in average F-measure and accuracy of 0.903 and 0.919 respectively.
 Deshmukh et al. \citep{DESHMUKH17} have proposed a new approach (siamese network) using a combination of CNNs and LSTMs to detect duplicate bug reports (features, results).
 Other research directions look at the bug duplicate detection problem from the perspective of semantic similarity and therefore employ topic modeling for the comparision of bug reports \citep{NEYSIANI19}, \citep{NGUYEN12}.
 Kim~\citep{KIM14} reported on the use of Convolutional Neural Networks on Sentence Classification tasks. He used different input representations, pre-trained word2vec and learning word2vec representations during the training and a combination of the two. The structure of the network was fairly simple, only one layer, and the hyperparameters were tuned for one of seven problems. In four out of seven cases CNN outperformed state of the art.
 Zhang and Wallace~\citep{ZHANG15}
 %Simese NN
Siamese neural networks have been used to resolved different problems in the software engineering domain.
Wehr et al. \citep{WEHR19} use siamese nn to construct semantic representations of source code based on which to detect code clones.
According to Wehr et al., the new representation outperforms simpler methods such as bag-of-tokens. % bag-of-words for NL
Zhao et al. \citep{ZHAO19} use siamese dense nn for the purpose of software defect prediction and report increased performance when compared to a benchmark of state-of-the-art approaches.
Siamese NN have also been used in several works to detect duplicate questions on software Q\&A websites \citep{IMTIAZ20}, \citep{GODBOLE18}.
 Heck and Zaidman~\cite{HECK2013} studied a set of 20 open-source GitHub projects, from which they highlighted the management of duplicated issues, as well as the visualization of the issue model and issue dependencies as two of the most critical challenges for software developers. However, these contributions are limited to providing general highlights to key challenges and features for issue management tasks, rather than designing and depicting concrete, detailed processes or theoretical models for the practical application of these features.


We want to use the existing approaches and generalize them to all types of relationships between issues. 


\section{Discussion}\label{sec:discussion}
% - Implication
% - Threats to Validity
\subsection{Implications}
A similar neural network architecture could be used for other problems where there are multiple types of inter-dependencies. Another approach in the need of testing is using two classifiers, the first testing if a inter-dependency is present and the second identifying the type of inter-dependency.
Another application could be the inter-dependency of software artifacts and issues.
Basically all applications where you have multiple types of connections between two objects, could be classified and identified in a similar fashion.


\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_0.png}
         \caption{No encoding}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_1.png}
         \caption{Encoding of description and title}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_2.png}
         \caption{Encoding of issues}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_3.png}
         \caption{Encoding of title, description and issues}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_7.png}
         \caption{Encoding of links}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_4.png}
         \caption{Encoding of issues and links}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_5.png}
         \caption{Encoding of title, description and links}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/model_6.png}
         \caption{Encoding of issues, title, description and link}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Model configurations}
        \label{fig:three graphs}
\end{figure*}

\subsection{Threats to Validity}
The inter-dependency type "No Inter-Dependency" was build on some assumptions on the correctness of the data. There could be human errors, we minimized this by making some assumptions and picking data accordingly. 
Furthermore, the data used in this work is by no means complete. In an earlier project, OpenReq\footnote{openreq.eu}, these missing and unknown inter-dependencies were explored and the challenge of finding these inter-dependencies was addressed. We also cannot make sure that all inter-dependencies are correct, but this is to be said for all data sets that are labeled by humans. 
We did not rigorously test all possible hyperparameter and network architectures (the amount of layers and layer parameters) combinations, so we can assume that results can be improved with more time and computing power. We tried to minimize the risk of wrong results due to that by sticking to heuristics for text classification for deep learning provided by Zhang et al.~\citep{ZHANG15}.

\section{Conclusion and Future Work}\label{sec:conclusion}
To conclude this work, we see the potential of this idea to improve identifying inter-dependencies and help organize issue tracking systems.
In the future, we want to test this approach more rigorously with more data sets and implement the classifier in a plug-in to find inter-dependencies between issues. Moreover, an implementation can help increase the quality and quantity of the data set.

\begin{table}[h!]
\caption{Qt. Simple Model. One vs. Rest}
\begin{center}
\begin{tabular}{ |r|l|l|l|l|l|l| } 
\hline
 Linktype & Prec. & Rec. & AUC & F1 & Acc. & Baseline\\
 \hline
 \multicolumn{7}{l}{Traditional}\\
 \hline
 Dependency         & 0.88 & 0.85 & 0.92 & 0.87 & 0.91 & +0.25\\
 Duplicate          & 0.71 & 0.66 & 0.79 & 0.68 & 0.86 & +0.10\\ 
 \hline
 \multicolumn{7}{l}{Cluster}\\
 \hline
Dependency & 0.49 & 0.49 & 0.49 & 0.49 & 0.62 & +0.01\\ 
Duplicate & 0.50 & 0.50 & 0.50 & 0.50 & 0.72 & +0.00\\ 
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\caption{Inteldaos. Simple Model. One vs. Rest.}
\begin{center}
\begin{tabular}{ |r|l|l|l|l|l|l| } 
\hline
 Linktype & Prec. & Rec. & AUC & F1 & Acc. & Baseline\\
 \hline
 \multicolumn{3}{l}{Traditional}\\
 \hline
 Duplicate          & 0.74 & 0.60 & 0.75 & 0.67 & 0.88 & +0.09\\
  \hline
 \multicolumn{3}{l}{Cluster}\\
 \hline
Duplicate & 0.41 & 0.46 & 0.46 & 0.44 & 0.78 & +0.04 \\ 
 \hline
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\caption{SecondLife. Simple Model. One vs. Rest.}
\begin{center}
\begin{tabular}{ |r|l|l|l|l|l|l| } 
\hline
 Linktype & Prec. & Rec. & AUC & F1 & Acc. & \\
 \hline
 \multicolumn{3}{l}{Traditional}\\
 \hline
 Depends            & 0.70 & 0.61 & 0.76 & 0.65 & 0.92 & +0.07\\
  \hline
 \multicolumn{3}{l}{Cluster}\\
 \hline
 Depends & 0.39 & 0.47 & 0.36 & 0.43 & 0.75 & -0.07 \\ 
 \hline
\end{tabular}
\end{center}
\end{table}

% Candidates to replicate:
% \begin{itemize}
%     \item Deshmukh et al.~\citep{DESHMUKH17}
%     \item \textbf{SiameseQAT: A Semantic Context-Based Duplicate Bug Report Detection Using Replicated Cluster Information}, 2018, sourcecode available
%     \item DWEN: deep word embedding network for duplicate bug report detection in software repositories, ICSE poster from 2020
%     \item Detecting Duplicate Bug Reports with Convolutional Neural Networks, 2018, no sourecode, but seems replicable 
%     \item Traceability Transformed: Generating more Accurate Links with Pre-Trained BERT Models, 2021, unsure because it is not between issues
%     \item Duplicate Bug Report Detection and Classification System Based on Deep Learning Technique, 2020
%     \item \textit{Blocking Bug Prediction Based on XGBoost with Enhanced Features}, 2020, interesting because other linktype
% 4    \item \textbf{Duplicate Bug Report Detection Using Dual-Channel Convolutional Neural Networks}, 2020, replicable
% \end{itemize}

If the correctly classified samples are already in the training set, the error is visible. Otherwise are they from clusters which are represented well in the training set? 

Possible consequence of wrong split: orphaned issues stay orphaned and connected components get more connected. ``Missing'' links in the original data do not get found or predicted when new issues are added.

\begin{table*}
\caption{Interesting Metrics - Overview}
 \begin{tabular}{|p{3cm} |p{4.5cm}| p{9.5cm} |}
\toprule
Name & What it means &  What it tells us \\
\midrule
Degree & How many links does an issue have on average / median / max / min / distribution / std.? & How connected is the graph? A high averages indicates that issues have a lot of links if they have links (include / exclude orphans) \\
\hline
Diameter & How ``long'' are the clusters? & A small diameter shows more tightly knit clusters, a high diameter means there are more line like \\
\hline
Effective Diameter & Length to include 90\% of all issues & To remove outliers from Diameter \\
\hline
Frequent Subgraphs & How often certain structures appear in the clusters & If there are a lot of triangles or V-shaped graphs this tells us something about the ``transitity'' of the clusters / linktypes. \\
\hline
Circle Detection & How many of the clusters contain circles? & If there are no circles, we have tree-like subgraphs \\
\hline
Density of clusters & How many edges are there in a certain cluster? & The denser the more links, connected to degree \\
\hline
Cyclomatic Complexity & How complex is the graph? & \\
\hline
Independnce Number & How many issues are there which have no links? & The higher the independence number, the less the connectedness\\
\hline
Largest Clique & How big is the largest clique & \\
\hline
Distribution of Clique sizes & how many cliques are there of which sizes & \\
\hline
Clustering coefficient & Number of Triangles times 3 divided by number of Vs & How clustered are the clusters?\\
\hline
Edit Distance ? && might not be applicable\\
\hline
Assortativity & How often ``strucutural similar'' issues are connected to each other & Social networks are more assortative, whereas technological networks are more disassortative\\
\hline
Tree Likeness ?  & & might be too complex\\
\hline
Average Degree of Neighbors & For each issues calculate how many links their linked issues possess & Are the subgraphs shaped like stars?\\
\hline
K-connectedness & How many links need to be removed to cut a graph into two components & If the average k is low, the clusters are very easily separated, might hint that there are links missing\\
\bottomrule
\end{tabular}
\end{table*}

Furthermore we used two ways of splitting the data:
\begin{itemize}
    \item[\textbf{Random}] The traditional split, we randomly sort the links and their respective issues in train and test set, e.g. if issue A and C are both linked to issue B, issue A and B could be in the train set and issue B and C in the test set. 
    \item[\textbf{Cluster}] We split the data randomly based on the underlying clusters, e.g. if issue A and C are both linked to issue B, all of them will be in the same set. 
\end{itemize}
If we split randomly we might introduce a bias in the test data. Some issues in the test set could already be in the training data and thus the test set is not totally unseen by the model.

%We found that ``General'' is different from the other link categories in its structure, the other link types consist of at least 93\% tree graphs, whereas ``Relate'' only has 82\% components that are without cycles. Thus this is a more ``clustered'' graph.
%``Incorporate'', ``Split'', and ``Cause'' consist mostly of star-shaped components, whereas ``Duplicate'', ``Clone'', and ``Block'' are rarely star-like. ``Duplicate'' and ``Clone'' are important to keep apart, as ``Duplicate'' links are unintentional duplicates and ``Clone'' links are intentional duplicates made by stakeholders, a detecting algorithm might not be able to distinguish them. Although ``Depend'' and ``Block'' are semantically very similar, Bugzilla uses the verbs to describe the same kind of link, they differ in the relative amount of stars found in them. ``Depend'' consists of more stars, which mean there are issues which depend on a lot of issues or issues which a lot of other issues depend on, other than that they are very similar.

%Figure~\ref{fig:LinkUsage} shows how often a specific link type was used in a project and Figure~\ref{fig:LinkComp} shows the link composition of the projects. We summarise the coloured link types as these are more common.
%\begin{itemize}
%    \item ``Relate'' is used the most and the most common, used in 33.5\% (RedHat) up to 63.8\% (Jira) of the links, average is 49.8\%. The percentage of involved issues in a project ranges from 1.7\% (Mindville) to 36.4\% (Jira).
%    \item ``Duplicate'' is used in all but one project (SecondLife), and is used from 6.6\% (RedHat) up to 37.0\% (Mindville) of the links, average is 18.1\%. The percentage of involved issues in a project ranges from 0.8\% (SonaType) to 12.8\% (MongoDB).
%    \item ``Clone'' is used from 0.1\% (Spring) up to 18.9\% (RedHat) of the links, average is 7.3\%. The percentage of involved issues in a project ranges from 0.04\% (Spring) to 9.4\% (RedHat).
%    \item ``Depend'' is used from 0.1\% (Jira) up to 26.0\% (Qt) of the links, average is 11.7\%. The percentage of involved issues in a project ranges from 0.04\% (Jira) to 10.0\% (MongoDB).
%    \item ``Incorporate'' is used from 2.3\% (JFrog) up to 11.3\% (RedHat) of the links, average is 6.0\%. The percentage of involved issues in a project ranges from 0.6\% (JFrog) to 4.6\% (MariaDB).
%    \item ``Split'' is used from 0.1\% (RedHat) up to 10.1\% (JFrog) of the links, average is 1.8\%. The percentage of involved issues in a project ranges from 0.01\% (SonaType) to 2.7\% (Qt).
 %   \item ``Block'' is used from 1.0\% (Jira) up to 26.0\% (Hyperledger) of the links, average is 14.1\%. The percentage of involved issues in a project ranges from 0.2\% (MindVille) to 7.6\% (RedHat).
%\end{itemize}


% \begin{table}
% \caption{Comparison of Link Ranking by how many projects use it and how often}\label{tab:LinkComp}
% \begin{tabular}{|l|ll|}
% \hline
%       Link type & Rank by Usage & Rank by Frequency \\
% \hline
%     Relate      & 1 & 1\\
%     Duplicate   & 2 & 2 \\
%     Clone       & 3 & 5 \\
%     Depend      & 4 & 4 \\
%     Incorporate & 5 & 6 \\
%     Split       & 6 & 7 \\
%     Block       & 7 & 3 \\
    
% \hline
% \end{tabular}
% \end{table}



%\begin{table}[h]
%    \centering
%    \caption{Cross / Same projects Links}
%    \label{tab:SameCrossProjectsLinkTypes}
%    \begin{tabular}{|l|rr|}
%    \hline
%\textbf{Link Type} & \textbf{\%SameProject}  & \textbf{\%CrossProject} \\
%         \hline
%\textbf{Relate}    &  88.9\% &    11.1\% \\
%\textbf{Duplicate}    &  96.8\% &    3.2\% \\
%\textbf{Clone}  &  85.7\% &    14.3\% \\
%\textbf{Depend} &  84.9\% &    15.1\% \\
%\textbf{Block}   &  88.0\% &    12.0\% \\
%\textbf{Incorporate}  &  94.2\% &    5.8\% \\
%\textbf{Split}   &  94.2\% &    5.8\% \\
%\textbf{Cause}    & 86.8\% &    13.2\% \\
%\hline
%    \end{tabular}
%\end{table}

%Table~\ref{tab:SameCrossProjectsLinkTypes} shows the share of same and cross projects links by link type. We see that ``Duplicate'', ``Incorporate'', and ``Split'' are more often found in the same project, whereas the others tend to be more across two projects.

% \begin{table}
% \caption{Usage of Links in Bugzilla}\label{tab:BugzillaStats}
% \begin{tabular}{|l|rrrr|}
% \hline
%     \textbf{Source}      & \textbf{Blocks}    & \textbf{Depends on}    & \textbf{Duplicate} &  \textbf{\#Issues} \\
% \hline
%     Eclipse     & 43251     & 29251        & 57559     & 561955 \\
%     NetBeans    & 14651   &  8752         & 39124     & 262011 \\
%     OpenOffice  & 6600     &  2299      & 20703   & 128343 \\
% \hline
% \end{tabular}
% \end{table}

%  Eclipse     & 43251 (7.7\%)     & 29251 (5.2\%)         & 57559 (10.2\%)    & 561955 \\
%     NetBeans    & 14651 (5.6\%)    &  8752 (3.3\%)        & 39124 (14.9\%)    & 262011 \\
%     OpenOffice  & 6600 (5.1\%)     &  2299 (1.8\%)        & 20703 (16.1\%)    & 128343 \\

% @article{WEHR19,
%   title={Learning Semantic Vector Representations of Source Code via a Siamese Neural Network},
%   author={David Wehr and Halley Fede and Eleanor Pence and Bo Zhang and Guilherme Ferreira and John Walczyk and Joseph Hughes},
%   journal={ArXiv},
%   year={2019},
%   volume={abs/1904.11968}
% }

% @article{Zhao:ACCESS:2019,
%     author={L. {Zhao} and Z. {Shang} and L. {Zhao} and A. {Qin} and Y. Y. {Tang}}, 
%     journal={IEEE Access}, 
%     title={Siamese Dense Neural Network for Software Defect Prediction With Small Data},
%     year={2019}, 
%     volume={7}, 
%     number={}, 
%     pages={7663-7677},
% }


% @article{IMTIAZ20, 
%     author={Z. {Imtiaz} and M. {Umer} and M. {Ahmad} and S. {Ullah} and G. S. {Choi} and A. {Mehmood}}, 
%     journal={IEEE Access}, 
%     title={Duplicate Questions Pair Detection Using Siamese MaLSTM},
%     year={2020},
%     volume={8}, 
%     number={}, 
%     pages={21932-21942},
% }

% @article{GODBOLE18,
%     author = {Godbole, Ameya and Dalmia, Aman and Sahu, Sunil},
%     year = {2018},
%     month = {01},
%     pages = {},
%     title = {Siamese Neural Networks with Random Forest for detecting duplicate question pairs}
% }

@inproceedings{KIM14,
    title = "Convolutional Neural Networks for Sentence Classification",
    author = "Kim, Yoon",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D14-1181",
    doi = "10.3115/v1/D14-1181",
    pages = "1746--1751",
}

@article{ZHANG15,
  author    = {Ye Zhang and
               Byron C. Wallace},
  title     = {A Sensitivity Analysis of (and Practitioners' Guide to) Convolutional
               Neural Networks for Sentence Classification},
  journal   = {CoRR},
  volume    = {abs/1510.03820},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.03820},
  archivePrefix = {arXiv},
  eprint    = {1510.03820},
  timestamp = {Mon, 13 Aug 2018 16:47:49 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ZhangW15b.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{CAMACHO_COLLADOS18,
    title = "On the Role of Text Preprocessing in Neural Network Architectures: An Evaluation Study on Text Categorization and Sentiment Analysis",
    author = "Camacho-Collados, Jose  and
      Pilehvar, Mohammad Taher",
    booktitle = "Proceedings of the 2018 {EMNLP} Workshop {B}lackbox{NLP}: Analyzing and Interpreting Neural Networks for {NLP}",
    month = nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W18-5406",
    doi = "10.18653/v1/W18-5406",
    pages = "40--46",
    abstract = "Text preprocessing is often the first step in the pipeline of a Natural Language Processing (NLP) system, with potential impact in its final performance. Despite its importance, text preprocessing has not received much attention in the deep learning literature. In this paper we investigate the impact of simple text preprocessing decisions (particularly tokenizing, lemmatizing, lowercasing and multiword grouping) on the performance of a standard neural text classifier. We perform an extensive evaluation on standard benchmarks from text categorization and sentiment analysis. While our experiments show that a simple tokenization of input text is generally adequate, they also highlight significant degrees of variability across preprocessing techniques. This reveals the importance of paying attention to this usually-overlooked step in the pipeline, particularly when comparing different models. Finally, our evaluation provides insights into the best preprocessing practices for training word embeddings.",
}

@inproceedings{NGUYEN15,
    title = "Relation Extraction: Perspective from Convolutional Neural Networks",
    author = "Nguyen, Thien Huu  and
      Grishman, Ralph",
    booktitle = "Proceedings of the 1st Workshop on Vector Space Modeling for Natural Language Processing",
    month = jun,
    year = "2015",
    address = "Denver, Colorado",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W15-1506",
    doi = "10.3115/v1/W15-1506",
    pages = "39--48",
}

@article{Zhang::2020,
	title = {{iLinker}: a novel approach for issue knowledge acquisition in {GitHub} projects},
	volume = {23},
	issn = {1573-1413},
	url = {https://doi.org/10.1007/s11280-019-00770-1},
	doi = {10.1007/s11280-019-00770-1},
	number = {3},
	journal = {World Wide Web},
	author = {Zhang, Yang and Wu, Yiwen and Wang, Tao and Wang, Huaimin},
	month = may,
	year = {2020},
	pages = {1589--1619},
}
% Table~\ref{tab:BugzillaStats} shows how often an issue had at least one other issue in the corresponding field. 
% ``Duplicate'' links appear more often than the other link types in Bugzilla, one reason could be that this link type is bound to the status property.
% often times creating link types that differ only a bit or nothing at all, Apache uses "Dependency" and "Dependent" 
% They have in common the high use of the link types \rel{} (35.3\%), \sub{} (20.6\%), \dup{} (13.3\%), and \epi{} (19.0\%). 
% We observed that \blo{} and \dep{} are used almost complementary, ITS with \blo{} links usually did not make use of \dep{} links and vice-versa, with the only exception being Apache. 
% This is also the case for \spl{} and \inc{}. 

% For instance, \Com{} presented a highly hierarchical structure, the exception to these might point to an inconsistency in the system.
% \Com{} links seem to be highly hierarchical in comparison to the other categories.
% The most common pattern seems to be one umbrella issue with at least two children issues.
% \Gen{} and \Wor{} are contain more cylces than other link categories.
% \Dup{} links are the simplest substructures, mostly consisting of issue pairs that are only connected to each other (82.8\% of all components) with a low density.
% \Tem{} and \Com{} tend to be larger substructures with more than three different issues connected to each other.

% Table~\ref{tab:DvsOLResults} shows the performance when we tasked the models to distinguish between \Dup{} and \OL{}. 
% The bad performance on the traditional test set is expected, as \NL{} were not in the training set, but the performance on the new test set is not better than for the DvsNL setting.

% \input{tables/model_results_DvsOL}



% Table~\ref{tab:ModelResults} shows the results of the SCCNN and DCCNN models.
% Our results show that the SCCNN model trained on DvsNL was not able to successfully distinguish \OL{} from \Dup{} in the traditional case, as the F1-score is 0.52. 
% This improved, once we added the \OL{} to the training set as attested by the results of DvsOL. 
% Still, even when we mixed the \OL{} with the \NL{} in DvsOLNL, the F1-Score was only 0.70, and the macro average was 0.69. 
% Once we trained the model to identify Links from \NL{} in DOLvsNL, we achieved the highest accuracy, ROC-AUC scores, and F1-scores reaching 0.74, 0.82, and 0.72 respectively.





% \input{tables/avg_model_results}
% Figure~\ref{fig:SCCNNF1} shows the SCCNN model performance for each training set combination on each project. 
% The models are ordered by number of links.
% We observe that the model always performed best on the DOLvsNL training set, except for ITS that contain a lower amount of links, such as JFrog, Hyperledger, and IntelDAOS, where the macro F1 score and accuracy was worse. 
% Overall, the DOLvsNL training set always seems to be the best choice for the larger ITS.

% \input{figures/SCCNN_performance}

% \input{figures/model_performance}

% The second half of Table~\ref{tab:ModelResults} shows the results of the DCCNN model. 
% The trend we observed in the SCCNN model is not evident for this model. 
% The difference between the metrics is smaller. 
% We observe that the model trained on the DvsOLNL set also performs well, on par with the DvsNL and DOLvsNL set.

% Figure~\ref{fig:DCCNNF1} shows the DCCNN model performance for each training set combination on each project. 
% Here, we see that only for two projects, Apache and Jira, the model learns better on the DOLvsNL train set.
% For RedHat, Sakai, Hyperledger, and JiraEcosystem the performance is better on the traditional DvsNL dataset. 
% For the other projects, the performance is about the same.
% We also observe that the DvsNLOL training set combination can improve the results for duplicate detection.

% \input{figures/DCCNN_performance}


% To test our hypothesis we conducted Welch's t-test on the results (macro F1, accuracy, and ROC-AUC) of the SCCNN and DCCNN model as suggested by Dietterich~\citep{Dietterich1998Approximate}.
% As we tested on 11 and 9 different projects respectively, the results stem from independent distributions and thus we can conduct a t-test. 
% As the variance of the results is different, we chose Welch's t-test as the Student's t-test assumes that the variance of the distributions is the same. 
% Our hypothesis is that the samples are drawn from different populations and thus we have a significant difference between the means. 
% Table~\ref{tab:WelchsTTest} shows the results. 
% As we can see we can only reject the hypothesis for the SCCNN model for accuracy.

% As we only have 11 and 9 values respectively, it makes sense to conduct a larger study.

% \begin{table}[h]
%     \centering
%     \caption{Welch's t-test p-Values}
%     \label{tab:WelchsTTest}
%     \begin{tabular}{|l|rrr|}
%     \hline
%          \textbf{Model}&\textbf{Accuracy}&\textbf{ROC-AUC}&\textbf{Macro F1}\\
%          \hline
% SCCNN & 0.025 & 0.065 & 0.066 \\
% DCCNN & 0.615 & 0.463 & 0.862\\
% \hline
%     \end{tabular}
% \end{table}

% We conducted a McNemar's test on all ITS, as we always tested on the same test set and it has a low Type I error~\citep{Dietterich:NC:1998}. 
% The McNemar’s test evaluates if the trained models make the same errors. 
% The null hypothesis is that the two models (\Dup{} detection [DvsNL] and Link detection [DOLvsNL]) make the same type of errors. 
% % Essentially, this test compares the true positive rate and true negative rate of the two models on the same test set.
% For the SCCNN model the null hypothesis was rejected for all but three repositories, namely SecondLife, JFrog, and Hyperledger.
% For the DCCNN model the null hypothesis was rejected for seven projects, only Qt, Sakai, and MariaDB did not reject the hypothesis.

% Single-Channel approaches seem to be a good candidate for general link detection models.




==> tables/avg_model_results.tex <==
\begin{table*}[h!]
\caption{Single Channel CNN and Dual Channel CNN model results averaged over projects.}\label{tab:ModelResults}
\begin{center}
\begin{tabular}{|l|l||r|r|r|r|r||r|r|r|r|r|} 
\hline
 \multirow{2}{*}{\textbf{Train Set}} & \multirow{2}{*}{\textbf{Class}} & \multicolumn{5}{c||}{\textbf{Single Channel CNN Model}} & \multicolumn{5}{c|}{\textbf{Dual Channel CNN Model}}\\
 \cline{3-12}
   &  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Accuracy} & \textbf{AUC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Accuracy} & \textbf{AUC}\\
  \hline
 \multirow{4}{*}{DvsNL} & 
 Duplicate & 0.52 &    0.85 & 0.64 & 
 \multirow{4}{*}{0.67} & \multirow{4}{*}{0.80} & 
 0.51 &    0.70 & 0.59 & 
 \multirow{4}{*}{0.68} & \multirow{4}{*}{0.75} \\ 
 & Other-Link & 0.75 &    0.43 & 0.52 & &  
 & 0.65 &    0.56 & 0.59 & &\\
 & Non-Link & 0.83 &    0.75 & \textbf{0.78} &  & 
 & 0.72 &    0.78 & \textbf{0.75} &  &\\
\cline{2-5}\cline{8-10}
 & Macro avg & 0.70 &    0.68 & 0.65 & & 
 & 0.63 &    0.68 & 0.64  & &\\
 \hline
 
 \multirow{4}{*}{DvsOL} & 
 Duplicate & 0.47 &    0.84 & 0.60 & 
 \multirow{4}{*}{0.62} & \multirow{4}{*}{0.76} 
 & 0.48 &    0.75 & 0.58 & 
 \multirow{4}{*}{0.64} & \multirow{4}{*}{0.73}\\ 
 & Other-Link & 0.80 &    0.63 & 0.70 & & 
 & 0.73 &    0.68 & \textbf{0.70} & &\\
 & Non-Link & 0.71 &    0.41 & 0.49 &  &  
 & 0.66 &    0.49 & 0.56 &  &\\
\cline{2-5}\cline{8-10}
 & Macro avg & 0.66 &    0.62 & 0.60 & & 
 & 0.62 &    0.64 & 0.61 & &\\
 \hline
 
 \multirow{4}{*}{DvsOLNL} & 
 Duplicate & 0.55 &    0.81 & 0.66 & 
 \multirow{4}{*}{0.71} & \multirow{4}{*}{0.81} 
 & 0.54 &     0.70 & 0.61 & 
 \multirow{4}{*}{\textbf{0.70}} & \multirow{4}{*}{\textbf{0.76}}\\ 
 & Other-Link & 0.78 &    0.64 & 0.70 &  &  
 & 0.70 &     0.70 & \textbf{0.70} &  &\\
 & Non-Link & 0.78 &    0.68 & 0.72 &  &  
 & 0.70 &     0.70 & 0.69 &  &\\
\cline{2-5}\cline{8-10}
 & Macro avg &  0.70 &    0.71 & 0.69 & & 
 & \textbf{0.65} &     \textbf{0.70} & 0.67  & &\\
 \hline
 
 \multirow{4}{*}{DOLvsNL} & 
 Duplicate & 0.79 &    0.72 & \textbf{0.74} &
 \multirow{4}{*}{\textbf{0.74}} & \multirow{4}{*}{\textbf{0.82}} 
 & 0.71 &    0.66 & \textbf{0.68} &
 \multirow{4}{*}{0.68} & \multirow{4}{*}{\textbf{0.76}}\\ 
 & Other-Link & 0.78 &    0.69 & \textbf{0.73} & & 
 & 0.71 &    0.64 & 0.67 & & \\
 & Non-Link &  0.60 &    0.81 & 0.68 & & 
 & 0.52 &    0.73 & 0.61 & &\\
\cline{2-5}\cline{8-10}
 & Macro avg &  \textbf{0.72} &    \textbf{0.74} & \textbf{0.72}  & & 
 & \textbf{0.65} &    0.68 & \textbf{0.65}  & &\\
 \hline
\end{tabular}
\end{center}
\end{table*}

==> tables/graph_metrics.tex <==
\begin{table*}
\renewcommand*{\arraystretch}{1.25}
\caption{Graph Theory Metrics}\label{tab:GTMetrics}
 \begin{tabularx}{\textwidth}{l X X}
%  {|m{2.5cm} |m{4.25cm}| m{9.9cm} |}
\hline
\textbf{Name} & \textbf{Definition} &  \textbf{Implication} \\
\hline
 \rowcolor{hellgrau}\%Isolated & The share of issues without links. & A high number of isolated issues shows that most issues are without links and that the links are concentrated on a few issues.\\
 \rowcolor{white}\#2Comp & The amount of components with exactly two or more issues. & A high number of 2-issues-components shows that graph is fairly simple.\\
 \rowcolor{hellgrau}\#3mComp & The amount of components with exactly two or more issues. & A high number of 3-or-more-issue-components shows that the graph is rather complex.\\
 \rowcolor{white}\%Trees & How many of the components are tree graphs. & If the graph's components mostly consist tree graphs the issues can be ordered hierarchically.\\
 \rowcolor{hellgrau}\%Stars & How many of the components are star graphs. & A high percentage of star graphs shows that one issue is often a central issue, connecting to many other issues which do not have any connections among each other.\\
 \rowcolor{white}Assortativity~\citep{Newman2002Assortative} & Pearson correlation between the degree of nodes at both ends of each edge in the network. & This value is between -1 and 1. Social networks are more assortative (positive values), whereas technological and biological networks are more disassortative (negative values). Assortative networks are more robust to vertex removal. Disassortative networks often have strong hierarchical configurations with large nodes connecting smaller nodes.\\
% This coefficient is the Pearson correlation between the order (degree) of nodes at both ends of each link (edge) in the network. The result ranges from -1 (low degree nodes often connect high degree nodes) to 1 (nodes of equal or similar degree are often connected). Disassortative networks (r is significantly negative) are often those with strong hierarchical configurations with large nodes connecting smaller nodes, as in scale-free networks, while regular networks are often assortative.
 \rowcolor{hellgrau}Transitivity & 3 times the number of triangles divided by number of triads (two links that share one issue) & This value is between 0 and 1.  Transitivity measures the frequency of triangles. A number near 0 means the graph has low transitivity and a number near 1 means the graph has high transitivity. E.g.: if a link type has high transitivity, then if issue A is linked with issue B which is in turn linked to issue C, that the stakeholders also put the issue link A-C in the ITS.\\
% https://transportgeography.org/contents/methods/graph-theory-measures-indices/transitivity-graph/
 \rowcolor{white}Average Density & The average number of links in a cluster divided by the number of possible links. & A high average density indicated that the graph components are highly inter-connected. We calculate this only for components with three or more issues.  \\
\hline
\end{tabularx}
\end{table*}

==> tables/linkcat_in_projcets.tex <==
\begin{tabular}{lrrrrr}
\toprule
category &  Composition &  General Relation &  Duplication &  Temporal/Causal &  Workflow \\
source        &              &                   &              &                  &           \\
\midrule
Apache        &         42.4 &              28.5 &         11.9 &             13.9 &       3.2 \\
Hyperledger   &         67.8 &              17.1 &          6.8 &              8.3 &       0.0 \\
IntelDAOS     &         71.5 &              12.1 &          8.1 &              8.1 &       0.1 \\
JFrog         &         37.6 &              27.2 &         20.6 &              8.3 &       6.3 \\
Jira          &          5.1 &              63.9 &         24.5 &              2.9 &       3.5 \\
JiraEcosystem &         46.7 &              23.3 &         17.5 &             11.6 &       0.9 \\
MariaDB       &         20.6 &              51.1 &          9.4 &             19.0 &       - \\
Mindville     &          - &              43.2 &         54.5 &              2.3 &       - \\
MongoDB       &          8.3 &              49.1 &         17.6 &             20.3 &       4.8 \\
Qt            &         43.3 &              22.4 &         17.8 &             16.4 &       0.1 \\
RedHat        &         29.8 &              26.6 &         20.7 &             22.4 &       0.5 \\
Sakai         &         24.2 &              48.7 &         14.3 &             12.9 &       0.0 \\
SecondLife    &         58.6 &              29.4 &          7.6 &              4.4 &       - \\
Sonatype      &         31.3 &              38.8 &          7.9 &              8.9 &      13.1 \\
Spring        &         24.7 &              47.7 &         12.2 &             12.1 &       3.3 \\
\bottomrule
\end{tabular}

==> tables/linkcat_metrics/casualtemp_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Temporal / Causal''}
    \label{tab:CatMetricsCasualTemp}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Isolated}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       Apache &       95.0\% &      70.9\% &      29.1\% &         0.042 &         -0.023 &     0.537 &    89.0\% &    67.9\% \\
  Hyperledger &       93.4\% &      63.4\% &      36.6\% &         0.074 &         -0.116 &     0.514 &    81.5\% &    61.1\% \\
    IntelDAOS &       93.5\% &      59.1\% &      40.9\% &         0.038 &         -0.183 &     0.514 &    86.7\% &    57.8\% \\
        JFrog &       96.9\% &      83.1\% &      16.9\% &         0.032 &          0.089 &     0.572 &    94.1\% &    85.3\% \\
         Jira &       98.2\% &      79.7\% &      20.3\% &         0.019 &         -0.034 &     0.596 &    95.2\% &    83.9\% \\
JiraEcosystem &       95.0\% &      75.7\% &      24.3\% &         0.313 &          0.335 &     0.585 &    90.5\% &    71.1\% \\
      MariaDB &       89.1\% &      65.4\% &      34.6\% &         0.006 &         -0.116 &     0.520 &    89.5\% &    70.2\% \\
    Mindville &       99.9\% &     100.0\% &     100.0\% &         0.000 &            NaN &     0.000 &     0.0\% &     0.0\% \\
      MongoDB &       89.2\% &      65.1\% &      34.9\% &         0.029 &         -0.089 &     0.505 &    85.5\% &    60.8\% \\
           Qt &       95.0\% &      63.5\% &      36.5\% &         0.007 &         -0.184 &     0.471 &    88.9\% &    71.5\% \\
       RedHat &       89.2\% &      70.1\% &      29.9\% &         0.023 &         -0.036 &     0.543 &    88.8\% &    67.5\% \\
        Sakai &       92.8\% &      68.2\% &      31.8\% &         0.056 &         -0.141 &     0.522 &    88.0\% &    69.6\% \\
     Sonatype &       99.1\% &      84.3\% &      15.7\% &         0.020 &         -0.028 &     0.576 &    97.8\% &    84.8\% \\
       Spring &       96.0\% &      71.5\% &      28.5\% &         0.061 &         -0.097 &     0.558 &    89.8\% &    70.1\% \\
   SecondLife &       97.6\% &      82.3\% &      17.6\% &         0.000 &         -0.057 &     0.430 &   100.0\% &    33.3\% \\
       \hline
\textbf{Mean} &      94.7\% &      73.5\% &      33.2\% &         0.048 &         -0.049 &     0.496 &    84.4\% &    63.7\% \\
\textbf{Standard Dev.} &        3.5\% &      10.8\% &      20.1\% &         0.077 &          0.132 &     0.144 &    23.8\% &    21.7\% \\
    \end{tabular}
\end{table*}

==> tables/linkcat_metrics/component_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Component''}
    \label{tab:CatMetricsComponent}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Isolated}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       Apache &       87.8\% &      40.9\% &      59.1\% &         0.001 &         -0.120 &     0.377 &    96.6\% &    90.1\% \\
  Hyperledger &       56.9\% &      21.5\% &      78.5\% &         0.000 &         -0.155 &     0.318 &    99.0\% &    85.1\% \\
    IntelDAOS &       54.6\% &      14.7\% &      85.3\% &         0.000 &         -0.316 &     0.276 &   100.0\% &    90.3\% \\
        JFrog &       90.7\% &      60.9\% &      39.1\% &         0.000 &         -0.513 &     0.490 &   100.0\% &   100.0\% \\
         Jira &       97.4\% &      61.6\% &      38.4\% &         0.002 &         -0.088 &     0.487 &    95.5\% &    85.9\% \\
JiraEcosystem &       85.7\% &      29.5\% &      70.5\% &         0.004 &         -0.324 &     0.379 &    96.0\% &    88.3\% \\
      MariaDB &       89.2\% &      49.7\% &      50.3\% &         0.005 &         -0.207 &     0.395 &    92.6\% &    81.2\% \\
      MongoDB &       96.2\% &      33.5\% &      66.5\% &         0.000 &         -0.207 &     0.368 &    99.6\% &    96.6\% \\
           Qt &       87.2\% &      52.6\% &      47.4\% &         0.001 &         -0.281 &     0.382 &    97.0\% &    82.8\% \\
       RedHat &       87.5\% &      43.0\% &      57.0\% &         0.002 &         -0.214 &     0.447 &    97.8\% &    91.2\% \\
        Sakai &       88.5\% &      55.5\% &      44.5\% &         0.005 &         -0.157 &     0.418 &    96.4\% &    88.6\% \\
     Sonatype &       97.9\% &      32.4\% &      67.6\% &         0.000 &         -0.345 &     0.388 &   100.0\% &    99.4\% \\
       Spring &       93.8\% &      43.1\% &      56.9\% &         0.000 &         -0.270 &     0.396 &   100.0\% &    95.6\% \\
   SecondLife &       77.0\% &      37.7\% &      62.3\% &         0.002 &         -0.445 &     0.397 &    97.4\% &    86.8\% \\
     \hline
\textbf{Mean} &       85.0\% &      41.2\% &      58.8\% &         0.002 &         -0.260 &     0.394 &    97.7\% &    90.1\% \\
\textbf{Standard Dev.} &       13.5\% &      14.1\% &      14.1\% &         0.002 &          0.121 &     0.057 &     2.2\% &     5.9\% \\
\hline
    \end{tabular}
\end{table*}

==> tables/linkcat_metrics/duplicate_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Duplication''}
    \label{tab:CatMetricsDuplicate}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Isolated}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
Apache &       94.7\% &      85.3\% &      14.7\% &         0.032 &         -0.011 &     0.607 &    95.9\% &    85.0\% \\
  Hyperledger &       93.3\% &      77.7\% &      22.3\% &         0.013 &         -0.025 &     0.579 &    97.6\% &    74.6\% \\
    IntelDAOS &       92.4\% &      81.2\% &      18.8\% &         0.045 &          0.306 &     0.583 &    93.3\% &    73.3\% \\
        JFrog &       91.8\% &      85.5\% &      14.5\% &         0.112 &         -0.012 &     0.640 &    93.8\% &    90.0\% \\
         Jira &       86.1\% &      70.7\% &      29.3\% &         0.058 &         -0.071 &     0.555 &    91.0\% &    77.0\% \\
JiraEcosystem &       91.9\% &      80.9\% &      19.1\% &         0.028 &         -0.047 &     0.592 &    95.9\% &    88.0\% \\
      MariaDB &       92.4\% &      79.2\% &      20.9\% &         0.115 &         -0.043 &     0.616 &    91.9\% &    83.9\% \\
    Mindville &       97.8\% &     100.0\% &       4.2\% &         0.000 &            NaN &     0.000 &     0.0\% &     0.0\% \\
      MongoDB &       87.7\% &      76.8\% &      23.2\% &         0.021 &         -0.058 &     0.575 &    97.3\% &    84.9\% \\
           Qt &       92.4\% &      76.1\% &      23.9\% &         0.046 &         -0.058 &     0.589 &    94.8\% &    84.1\% \\
       RedHat &       87.9\% &      82.9\% &      17.1\% &         0.109 &          0.050 &     0.613 &    90.1\% &    70.9\% \\
        Sakai &       90.4\% &      83.1\% &      16.9\% &         0.063 &         -0.027 &     0.599 &    93.3\% &    76.5\% \\
     Sonatype &       99.2\% &      90.6\% &       9.4\% &         0.064 &          0.021 &     0.636 &    96.4\% &    89.3\% \\
       Spring &       95.4\% &      84.7\% &      15.3\% &         0.047 &         -0.071 &     0.613 &    95.8\% &    88.5\% \\
   SecondLife &       95.3\% &      87.2\% &      12.8\% &         0.000 &          0.084 &     0.567 &   100.0\% &    80.0\% \\
       \hline
\textbf{Mean} &       92.6\% &      82.8\% &      17.5\% &         0.050 &          0.003 &     0.558 &    88.5\% &    76.4\% \\
\textbf{Standard Dev.} &         3.6\% &       6.9\% &       6.2\% &         0.038 &          0.098 &     0.156 &    24.6\% &    22.0\% \\
\hline
    \end{tabular}
\end{table*}

==> tables/linkcat_metrics/related_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``General''}
    \label{tab:CatMetricsRelated}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Isolated}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       Apache &       89.8\% &      68.8\% &      31.1\% &         0.100 &         -0.016 &     0.557 &    83.0\% &    59.8\% \\
  Hyperledger &       87.2\% &      62.1\% &      37.9\% &         0.163 &         -0.051 &     0.534 &    79.0\% &    60.4\% \\
    IntelDAOS &       90.2\% &      56.3\% &      43.7\% &         0.080 &         -0.171 &     0.533 &    81.6\% &    60.5\% \\
        JFrog &       90.3\% &      74.1\% &      25.9\% &         0.111 &          0.070 &     0.593 &    87.8\% &    65.5\% \\
         Jira &       63.8\% &      87.7\% &      12.3\% &         0.133 &          0.203 &     0.559 &    62.3\% &    45.5\% \\
JiraEcosystem &       90.3\% &      73.8\% &      26.2\% &         0.452 &          0.609 &     0.592 &    85.9\% &    69.4\% \\
      MariaDB &       74.4\% &      63.8\% &      36.2\% &         0.098 &         -0.040 &     0.563 &    71.9\% &    52.0\% \\
    Mindville &       98.4\% &      87.5\% &      12.5\% &         0.000 &         -0.137 &     0.583 &   100.0\% &   100.0\% \\
      MongoDB &       76.5\% &      63.8\% &      36.2\% &         0.028 &          0.088 &     0.544 &    81.0\% &    55.0\% \\
           Qt &       91.5\% &      71.6\% &      28.4\% &         0.099 &         -0.028 &     0.566 &    83.3\% &    60.9\% \\
       RedHat &       86.9\% &      69.9\% &      30.1\% &         0.098 &         -0.011 &     0.568 &    82.4\% &    61.3\% \\
        Sakai &       76.7\% &      64.1\% &      35.9\% &         0.073 &         -0.046 &     0.538 &    77.8\% &    52.3\% \\
     Sonatype &       96.5\% &      76.4\% &      23.6\% &         0.160 &          0.015 &     0.598 &    86.0\% &    69.7\% \\
       Spring &       86.9\% &      67.6\% &      32.4\% &         0.148 &          0.014 &     0.555 &    80.4\% &    57.9\% \\
   SecondLife &       84.7\% &      72.1\% &      27.9\% &         0.069 &         -0.123 &     0.547 &    86.2\% &    72.4\% \\
       \hline
         \textbf{Mean} &       85.6\% &      70.7\% &      29.3\% &         0.121 &          0.025 &     0.562 &    81.9\% &    62.8\% \\
\textbf{Standard Dev.} &        9.1\% &       8.7\% &       8.7\% &         0.102 &          0.186 &     0.022 &     8.2\% &    12.6\% \\
\hline
    \end{tabular}
\end{table*}

==> tables/linkcat_metrics/seactivity_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Activity''}
    \label{tab:CatMetricsActivity}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Isolated}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       Apache &       98.6\% &      83.6\% &      16.4\% &         0.005 &         -0.015 &     0.597 &    97.4\% &    87.4\% \\
  Hyperledger &      100.0\% &      83.3\% &      16.7\% &         0.000 &         -0.167 &     0.667 &   100.0\% &   100.0\% \\
    IntelDAOS &       99.9\% &     100.0\% &      33.3\% &         0.000 &            NaN &     0.000 &     0.0\% &     0.0\% \\
        JFrog &       97.4\% &      89.3\% &      10.7\% &         0.000 &         -0.080 &     0.618 &   100.0\% &    94.7\% \\
         Jira &       98.0\% &      70.4\% &      29.6\% &         0.004 &         -0.114 &     0.534 &    98.8\% &    94.4\% \\
JiraEcosystem &       99.6\% &      72.3\% &      27.7\% &         0.000 &         -0.191 &     0.560 &   100.0\% &    83.3\% \\
      MongoDB &       96.3\% &      93.3\% &       6.7\% &         0.000 &         -0.012 &     0.588 &    99.1\% &    81.5\% \\
           Qt &       99.9\% &      80.0\% &      20.0\% &         0.000 &         -0.179 &     0.571 &   100.0\% &   100.0\% \\
       RedHat &       99.7\% &      76.8\% &      23.2\% &         0.000 &         -0.091 &     0.591 &    98.8\% &    93.9\% \\
        Sakai &      100.0\% &     100.0\% &     100.0\% &         0.000 &            NaN &     0.000 &     0.0\% &     0.0\% \\
     Sonatype &       98.7\% &      82.4\% &      17.6\% &         0.026 &         -0.024 &     0.579 &    97.3\% &    78.4\% \\
       Spring &       98.8\% &      83.2\% &      16.8\% &         0.000 &         -0.110 &     0.575 &    98.4\% &    93.5\% \\
       \hline
\textbf{Mean} &       98.9\% &      84.5\% &      26.6\% &         0.003 &         -0.098 &     0.490 &    82.5\% &    75.6\% \\
\textbf{Standard Dev.} &        1.2\% &       9.6\% &      24.4\% &         0.007 &          0.067 &     0.231 &    38.5\% &    36.0\% \\
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_categories.tex <==
\begin{table*}
\renewcommand*{\arraystretch}{1.25}
\caption{Link Type Categories}\label{tab:LinkTypeCat}
 \begin{tabular}{|m{3cm} |m{13.75cm}|}
\hline
\textbf{Category} & \textbf{Definition}   \\
\hline
\textbf{\Gen{}} & Links which indicate a general relationship between issues, which is not specific, such as a logical or temporal dependency, structural component. E.g.: The same java class is the origin of the bug.  \\
\hline
\textbf{\Dup{}} & Links which indicate that an issue describes the same bug, feature, or task as another issue. This issue can be added intentional (Clone, Replace) or unintentional (Duplicate). E.g.: Two users found and submitted a ticked for the same bug without being aware that the bug was already documented in the ITS by another user. \\
\hline
\textbf{\Tem{}} & Links which indicate that an issue depends on the status of another issue. This can be due to causal or temporal reasons. E.g.: One feature is part of the release, a second feature which builds up on the first feature can only be released later. \\
\hline
\textbf{\Com{}} & Links which indicate a structural dependency between two issues. This link is created when an issue is split into multiple sub-issues or when user stories belong to an epic. E.g.: A stakeholder creates a ticket for a feature and splits it into multiple tasks that need to be completed. \\
\hline
\textbf{\Wor{}} & Links that indicate that an issue was discovered, reported, fixed, refined, or documents while working on a certain software engineering activity on another issue, like testing, reviewing changes, or implementing this issue.  E.g.: While testing a feature, a developer found an unknown bug and documented it. \\
\hline
\end{tabular}
\end{table*}

==> tables/linktype_metrics/block_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Block''}
    \label{tab:MetricsBlock}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       apache &       97.7\% &      72.4\% &      27.6\% &         0.018 &         -0.035 &     0.534 &    91.2\% &    72.7\% \\
  hyperledger &       93.1\% &      62.8\% &      37.2\% &         0.065 &         -0.123 &     0.512 &    80.8\% &    61.6\% \\
    inteldaos &       94.6\% &      59.6\% &      40.4\% &         0.025 &         -0.199 &     0.517 &    86.8\% &    57.9\% \\
         jira &       99.4\% &      83.2\% &      16.9\% &         0.007 &         -0.044 &     0.593 &    95.9\% &    85.1\% \\
jiraecosystem &       97.5\% &      77.2\% &      22.8\% &         0.446 &          0.424 &     0.598 &    90.6\% &    74.0\% \\
      mariadb &       92.6\% &      65.3\% &      34.7\% &         0.004 &         -0.159 &     0.520 &    90.8\% &    71.7\% \\
       redhat &       92.6\% &      71.3\% &      28.7\% &         0.017 &         -0.049 &     0.540 &    89.2\% &    69.9\% \\
       \hline
         Mean &       95.4\% &      70.2\% &      29.8\% &         0.083 &         -0.026 &     0.545 &    89.3\% &    70.4\% \\
Standard Dev. &        2.8\% &       8.3\% &       8.3\% &         0.161 &          0.208 &     0.036 &     4.6\% &     8.8\% \\
% hyperledger & 25992 & 370 & 219 & -0.12 & 0.06 &&&&\\
% redhat & 292492 & 5459 & 2201 & -0.05 & 0.02 &&&&\\
% inteldaos & 5256 & 56 & 38 & -0.2 & 0.02 &&&&\\
% mariadb & 28926 & 325 & 173 & -0.16 & 0.0 &&&&\\
% mindville & 2132 & 1 & 0 & - & 0.0 &&&&\\
% jira & 263676 & 597 & 121 & -0.04 & 0.01 &&&&\\
% jiraecosystem & 39578 & 325 & 96 & 0.42 & 0.45 &&&&\\
% apache & 948428 & 5567 & 2118 & -0.03 & 0.02 &&&&\\ %Checl
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/cause_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Cause''}
    \label{tab:MetricsCause}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
        apache &       99.5\% &      85.8\% &      14.2\% &         0.022 &         -0.037 &     0.599 &    97.5\% &    85.2\% \\
         jira &       98.8\% &      80.7\% &      19.3\% &         0.020 &         -0.055 &     0.604 &    96.1\% &    85.3\% \\
jiraecosystem &       98.2\% &      83.3\% &      16.7\% &         0.038 &          0.001 &     0.620 &    90.6\% &    84.9\% \\
      mariadb &       96.0\% &      71.0\% &      28.9\% &         0.020 &         -0.126 &     0.528 &    87.6\% &    72.7\% \\
      mongodb &       98.7\% &      85.8\% &      14.2\% &         0.010 &         -0.048 &     0.585 &    97.2\% &    76.4\% \\
       redhat &       98.4\% &      76.4\% &      23.6\% &         0.014 &         -0.078 &     0.578 &    95.6\% &    82.7\% \\
     sonatype &       99.5\% &      87.5\% &      12.5\% &         0.041 &         -0.050 &     0.590 &    95.7\% &    91.3\% \\
     \hline
         Mean &       98.5\% &      81.5\% &      18.5\% &         0.024 &         -0.056 &     0.586 &    94.3\% &    82.7\% \\
Standard Dev. &        1.2\% &       5.9\% &       5.9\% &         0.012 &          0.039 &     0.029 &     3.8\% &     6.2\% \\

\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/clone_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Clone''}
    \label{tab:MetricsClone}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       apache &       99.3\% &      87.9\% &      12.1\% &         0.008 &          0.088 &     0.556 &    99.0\% &    66.3\% \\
  hyperledger &       97.3\% &      73.7\% &      26.4\% &         0.000 &          0.174 &     0.534 &   100.0\% &    57.5\% \\
    inteldaos &       96.1\% &      84.5\% &      15.5\% &         0.000 &          0.399 &     0.472 &   100.0\% &    54.5\% \\
         jira &       98.1\% &      92.1\% &       7.9\% &         0.017 &          0.066 &     0.613 &    98.4\% &    85.9\% \\
jiraecosystem &       99.1\% &      88.4\% &      11.6\% &         0.094 &          0.174 &     0.616 &    94.7\% &    68.4\% \\
      mongodb &       99.9\% &      88.0\% &      12.0\% &         0.000 &          0.213 &     0.611 &   100.0\% &    83.3\% \\
       redhat &       90.8\% &      83.5\% &      16.5\% &         0.057 &          0.021 &     0.608 &    94.7\% &    75.1\% \\
        sakai &       96.9\% &      84.4\% &      15.6\% &         0.005 &         -0.045 &     0.530 &    99.0\% &    65.6\% \\
   secondlife &       95.2\% &      87.5\% &      12.5\% &         0.000 &          0.088 &     0.567 &   100.0\% &    80.0\% \\
   \hline
         Mean &       97.0\% &      85.5\% &      14.5\% &         0.020 &          0.131 &     0.567 &    98.4\% &    70.8\% \\
Standard Dev. &        2.8\% &       5.2\% &       5.2\% &         0.033 &          0.129 &     0.050 &     2.2\% &    11.1\% \\
% hyperledger & 27167 & 204 & 73 & 0.17 & 0.0 &&&&\\
% sakai & 47677 & 519 & 96 & -0.05 & 0.01 &&&&\\
% jfrog & 14729 & 20 & 0 & - & 0.0 &&&&\\
% redhat & 286612 & 10596 & 2098 & 0.02 & 0.06 &&&&\\
% inteldaos & 5341 & 60 & 11 & 0.4 & 0.0 &&&&\\
% mongodb & 90520 & 44 & 6 & 0.21 & 0.0 &&&&\\
% secondlife & 1776 & 35 & 5 & 0.09 & 0.0 &&&&\\
% mindville & 2120 & 7 & 0 & - & 0.0 &&&&\\
% jira & 260214 & 2229 & 192 & 0.07 & 0.02 &&&&\\
% jiraecosystem & 40246 & 145 & 19 & 0.17 & 0.09 &&&&\\
% spring & 69072 & 14 & 0 & - & 0.0 &&&&\\
% apache & 963525 & 2774 & 382 & 0.09 & 0.01 &&&&\\ %Check
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/depend_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Depend''}
    \label{tab:MetricsDepend}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       apache &       98.0\% &      73.7\% &      26.3\% &         0.084 &          0.046 &     0.553 &    89.5\% &    71.9\% \\
        jfrog &       97.0\% &      82.9\% &      17.1\% &         0.032 &          0.087 &     0.569 &    93.9\% &    84.8\% \\
         jira &      100.0\% &      85.7\% &      14.3\% &         0.000 &         -0.134 &     0.594 &   100.0\% &   100.0\% \\
jiraecosystem &       99.5\% &      72.4\% &      27.6\% &         0.060 &         -0.136 &     0.593 &    95.8\% &    83.3\% \\
      mongodb &       90.2\% &      64.3\% &      35.7\% &         0.029 &         -0.095 &     0.501 &    85.1\% &    61.1\% \\
           qt &       95.0\% &      63.6\% &      36.4\% &         0.007 &         -0.185 &     0.472 &    88.7\% &    71.8\% \\
        sakai &       92.7\% &      67.9\% &      32.1\% &         0.058 &         -0.142 &     0.521 &    87.9\% &    69.8\% \\
   secondlife &       97.5\% &      83.3\% &      16.7\% &         0.000 &         -0.049 &     0.430 &   100.0\% &    33.3\% \\
     sonatype &       99.6\% &      85.4\% &      14.6\% &         0.000 &          0.012 &     0.557 &   100.0\% &    77.8\% \\
       spring &       96.0\% &      71.5\% &      28.5\% &         0.063 &         -0.097 &     0.558 &    89.5\% &    69.9\% \\
       \hline
         Mean &       96.5\% &      75.1\% &      24.9\% &         0.033 &         -0.069 &     0.535 &    93.0\% &    72.4\% \\
Standard Dev. &        3.2\% &       8.6\% &       8.6\% &         0.031 &          0.090 &     0.053 &     5.6\% &    17.4\% \\
% qt & 133168 & 929 & 532 & -0.18 & 0.01 &&&&\\
% sakai & 45612 & 817 & 387 & -0.14 & 0.06 &&&&\\
% jfrog & 14325 & 160 & 33 & 0.09 & 0.03 &&&&\\
% mongodb & 81767 & 1553 & 861 & -0.1 & 0.03 &&&&\\
% secondlife & 1818 & 15 & 3 & -0.05 & 0.0 &&&&\\
% sonatype & 77551 & 105 & 18 & 0.01 & 0.0 &&&&\\
% jira & 265249 & 36 & 6 & -0.13 & 0.0 &&&&\\
% jiraecosystem & 40391 & 63 & 24 & -0.14 & 0.06 &&&&\\
% spring & 66347 & 741 & 296 & -0.1 & 0.06 &&&&\\
% apache & 951755 & 5022 & 1795 & 0.05 & 0.08 &&&&\\ %check
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/duplicate_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Duplicate''}
    \label{tab:MetricsDuplicate}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       apache &       95.4\% &      85.7\% &      14.3\% &         0.026 &         -0.012 &     0.611 &    96.3\% &    88.8\% \\
  hyperledger &       95.9\% &      82.7\% &      17.3\% &         0.027 &         -0.059 &     0.618 &    96.6\% &    90.9\% \\
    inteldaos &       96.2\% &      79.6\% &      20.4\% &         0.100 &         -0.067 &     0.644 &    94.7\% &    94.7\% \\
        jfrog &       92.0\% &      85.3\% &      14.7\% &         0.092 &         -0.026 &     0.635 &    94.9\% &    91.1\% \\
         jira &       87.7\% &      69.0\% &      30.9\% &         0.038 &         -0.083 &     0.549 &    92.9\% &    79.9\% \\
jiraecosystem &       92.7\% &      80.8\% &      19.2\% &         0.022 &         -0.051 &     0.592 &    95.8\% &    91.7\% \\
      mariadb &       92.4\% &      79.2\% &      20.9\% &         0.115 &         -0.043 &     0.616 &    91.9\% &    83.9\% \\
      mongodb &       87.8\% &      76.8\% &      23.2\% &         0.019 &         -0.059 &     0.575 &    97.2\% &    85.0\% \\
           qt &       95.3\% &      77.2\% &      22.8\% &         0.067 &         -0.053 &     0.603 &    93.6\% &    85.9\% \\
       redhat &       96.8\% &      89.2\% &      10.8\% &         0.091 &          0.028 &     0.632 &    92.5\% &    85.8\% \\
        sakai &       93.3\% &      85.1\% &      14.9\% &         0.071 &         -0.043 &     0.622 &    94.5\% &    85.9\% \\
     sonatype &       99.2\% &      90.6\% &       9.4\% &         0.060 &          0.032 &     0.634 &    96.4\% &    89.3\% \\
       spring &       95.5\% &      84.6\% &      15.4\% &         0.047 &         -0.071 &     0.614 &    95.8\% &    88.9\% \\
       \hline
         Mean &       93.9\% &      82.0\% &      18.0\% &         0.060 &         -0.039 &     0.611 &    94.9\% &    87.8\% \\
Standard Dev. &        3.4\% &       5.8\% &       5.8\% &         0.033 &          0.036 &     0.026 &     1.7\% &     3.9\% \\
% qt & 133716 & 2116 & 624 & -0.05 & 0.07 & & & & \\
% hyperledger & 26766 & 421 & 88 & -0.06 & 0.03 & & & & \\
% sakai & 45933 & 1256 & 220 & -0.04 & 0.07  & & & & \\
% jfrog & 13592 & 459 & 79 & -0.03 & 0.09  & & & & \\
% redhat & 305709 & 4185 & 506 & 0.03 & 0.09  & & & & \\
% inteldaos & 5348 & 74 & 19 & -0.07 & 0.1  & & & & \\
% mongodb & 79571 & 3483 & 1053 & -0.06 & 0.02  & & & & \\
% mariadb & 28864 & 801 & 211 & -0.04 & 0.11  & & & & \\
% mindville & 2100 & 17 & 0 & - & 0.0  & & & & \\
% sonatype & 77198 & 271 & 28 & 0.03 & 0.06  & & & & \\
% jira & 232808 & 8069 & 3616 & -0.08 & 0.04  & & & & \\
% jiraecosystem & 37644 & 1010 & 240 & -0.05 & 0.02  & & & & \\
% spring & 65956 & 1191 & 217 & -0.07 & 0.05  & & & & \\
% apache & 925694 & 17308 & 2895 & -0.01 & 0.03  & & & & \\ %Check
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/incorporate_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Incorporate''}
    \label{tab:MetricsIncorporate}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
        apache &       98.5\% &      72.8\% &      27.2\% &         0.006 &         -0.100 &     0.506 &    95.8\% &    87.2\% \\
        jfrog &       99.4\% &      92.3\% &       7.7\% &         0.000 &         -0.094 &     0.556 &   100.0\% &   100.0\% \\
         jira &       98.6\% &      70.5\% &      29.5\% &         0.010 &         -0.065 &     0.531 &    92.9\% &    78.5\% \\
jiraecosystem &       99.2\% &      81.2\% &      18.8\% &         0.000 &         -0.122 &     0.557 &   100.0\% &    92.6\% \\
      mariadb &       95.4\% &      63.2\% &      36.8\% &         0.008 &         -0.203 &     0.474 &    91.0\% &    79.3\% \\
       redhat &       96.0\% &      63.2\% &      36.8\% &         0.006 &         -0.140 &     0.491 &    93.8\% &    76.6\% \\
        sakai &       96.2\% &      74.4\% &      25.6\% &         0.004 &         -0.092 &     0.515 &    94.9\% &    84.6\% \\
   secondlife &       98.8\% &      71.4\% &      28.6\% &         0.000 &         -0.410 &     0.375 &   100.0\% &   100.0\% \\
   \hline
         Mean &       97.8\% &      73.6\% &      26.4\% &         0.004 &         -0.153 &     0.501 &    96.1\% &    87.3\% \\
Standard Dev. &        1.6\% &       9.6\% &       9.6\% &         0.004 &          0.112 &     0.059 &     3.6\% &     9.4\% \\
% sakai & 47341 & 454 & 155 & -0.09 & 0.0 &&&&\\
% jfrog & 14686 & 36 & 3 & -0.09 & 0.0 &&&&\\
% redhat & 303296 & 2008 & 1168 & -0.14 & 0.01 &&&&\\
% mariadb & 29804 & 191 & 111 & -0.2 & 0.01 &&&&\\
% secondlife & 1843 & 5 & 2 & -0.41 & 0.0 &&&&\\
% jira & 261659 & 911 & 381 & -0.07 & 0.01 &&&&\\
% jiraecosystem & 40255 & 117 & 27 & -0.12 & 0.0 &&&&\\
% apache & 955693 & 3505 & 1312 & -0.1 & 0.01 &&&&\\ %Check
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/overview_avg.tex <==
\begin{table*}[h]
    \centering
    \caption{Comparison Link Types}
    \label{tab:MetricsComparison}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
\textbf{Relate}    &      85.5\% &      70.3\% &      29.7\% &         0.121 &          0.022 &     0.561 &    81.8\% &    62.9\% \\
\textbf{Duplicate}    &    93.9\% &      82.0\% &      18.0\% &         0.060 &         -0.039 &     0.611 &    94.9\% &    87.8\% \\
\textbf{Clone}  &     97.0\% &      85.5\% &      14.5\% &         0.020 &          0.131 &     0.567 &    98.4\% &    70.8\% \\
\textbf{Depend} &       96.5\% &      75.1\% &      24.9\% &         0.033 &         -0.069 &     0.535 &    93.0\% &    72.4\% \\
\textbf{Block}  &     95.4\% &      70.2\% &      29.8\% &         0.083 &         -0.026 &     0.545 &    89.3\% &    70.4\% \\
\textbf{Incorporate} &      97.8\% &      73.6\% &      26.4\% &         0.004 &         -0.153 &     0.501 &    96.1\% &    87.3\% \\
\textbf{Split}  &     99.5\% &      72.8\% &      27.2\% &         0.001 &         -0.204 &     0.553 &    98.3\% &    88.5\% \\
\textbf{Cause}  &     98.5\% &      81.5\% &      18.5\% &         0.024 &         -0.056 &     0.586 &    94.3\% &    82.7\% \\
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/relate_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Relate''}
    \label{tab:MetricsRelate}
    \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
       apache &       89.8\% &      68.8\% &      31.2\% &         0.099 &         -0.016 &     0.557 &    83.0\% &    59.7\% \\
  hyperledger &       86.9\% &      61.6\% &      38.4\% &         0.156 &         -0.059 &     0.531 &    79.5\% &    60.2\% \\
    inteldaos &       90.1\% &      56.0\% &      44.0\% &         0.078 &         -0.177 &     0.530 &    81.8\% &    61.0\% \\
        jfrog &       90.3\% &      74.1\% &      25.9\% &         0.115 &          0.071 &     0.592 &    87.2\% &    65.1\% \\
         jira &       63.8\% &      87.7\% &      12.3\% &         0.133 &          0.203 &     0.559 &    62.3\% &    45.6\% \\
jiraecosystem &       90.3\% &      73.8\% &      26.2\% &         0.452 &          0.609 &     0.592 &    86.0\% &    69.2\% \\
      mariadb &       74.4\% &      63.9\% &      36.1\% &         0.097 &         -0.040 &     0.563 &    71.8\% &    52.0\% \\
    mindville &       98.4\% &      87.5\% &      12.5\% &         0.000 &         -0.137 &     0.583 &   100.0\% &   100.0\% \\
      mongodb &       76.5\% &      63.8\% &      36.2\% &         0.028 &          0.088 &     0.544 &    81.0\% &    55.0\% \\
           qt &       91.5\% &      71.5\% &      28.5\% &         0.098 &         -0.028 &     0.566 &    83.4\% &    61.1\% \\
       redhat &       86.9\% &      69.9\% &      30.1\% &         0.098 &         -0.011 &     0.567 &    82.3\% &    61.2\% \\
        sakai &       76.6\% &      63.9\% &      36.1\% &         0.074 &         -0.046 &     0.539 &    77.9\% &    52.5\% \\
   secondlife &       84.2\% &      68.3\% &      31.7\% &         0.075 &         -0.151 &     0.545 &    84.8\% &    72.7\% \\
     sonatype &       96.5\% &      76.3\% &      23.6\% &         0.160 &          0.014 &     0.598 &    86.0\% &    69.8\% \\
       spring &       86.9\% &      67.6\% &      32.4\% &         0.149 &          0.013 &     0.555 &    80.2\% &    57.8\% \\
       \hline
         Mean &       85.5\% &      70.3\% &      29.7\% &         0.121 &          0.022 &     0.561 &    81.8\% &    62.9\% \\
Standard Dev. &        9.1\% &       8.8\% &       8.8\% &         0.102 &          0.189 &     0.022 &     8.1\% &    12.6\% \\
         
% qt & 128261 & 3068 & 1221 & -0.03 & 0.1 & & & & \\
% hyperledger & 24259 & 651 & 405 & -0.06 & 0.16& & & & \\
% sakai & 37702 & 1891 & 1070 & -0.05 & 0.07& & & & \\
% jfrog & 13333 & 426 & 149 & 0.07 & 0.12& & & & \\
% redhat & 274297 & 10295 & 4441 & -0.01 & 0.1& & & & \\
% inteldaos & 5007 & 98 & 77 & -0.18 & 0.08& & & & \\
% mongodb & 69336 & 3723 & 2114 & 0.09 & 0.03& & & & \\
% mariadb & 23227 & 1170 & 662 & -0.04 & 0.1& & & & \\
% secondlife & 1570 & 71 & 33 & -0.15 & 0.08& & & & \\
% mindville & 2099 & 14 & 2 & -0.14 & 0.0& & & & \\
% sonatype & 75132 & 833 & 258 & 0.01 & 0.16& & & & \\
% jira & 169396 & 33874 & 4770 & 0.2 & 0.13& & & & \\
% jiraecosystem & 36661 & 1145 & 406 & 0.61 & 0.45& & & & \\
% spring & 60019 & 1837 & 881 & 0.01 & 0.15& & & & \\
% apache & 871718 & 22647 & 10271 & -0.02 & 0.1& & & & \\ %Check
\hline
    \end{tabular}
\end{table*}

==> tables/linktype_metrics/split_metrics.tex <==
\begin{table*}[h]
    \centering
    \caption{Metrics for ``Split''}
    \label{tab:MetricsSplit}
   \begin{tabular}{|l|rrrrrrrr|}
    \hline
\textbf{Project} & \textbf{\%Orphans}  & \textbf{\%2Comp} & \textbf{\%3>Comp} &  \textbf{Transitivity} & \textbf{Assortativity}& \textbf{Avg. Dense} &  \textbf{\%Trees} & \textbf{\%Star} \\
         \hline
   hyperledger &       99.6\% &      70.0\% &      30.0\% &         0.000 &         -0.210 &     0.470 &   100.0\% &    66.7\% \\
         jira &       99.9\% &      78.3\% &      21.6\% &         0.000 &         -0.157 &     0.548 &    90.5\% &    90.5\% \\
jiraecosystem &       99.5\% &      76.1\% &      23.9\% &         0.000 &         -0.182 &     0.569 &   100.0\% &    95.5\% \\
      mariadb &       99.9\% &      73.3\% &      26.7\% &         0.000 &         -0.212 &     0.542 &   100.0\% &    75.0\% \\
      mongodb &       99.8\% &      62.7\% &      37.3\% &         0.000 &         -0.322 &     0.504 &   100.0\% &    96.0\% \\
           qt &       97.3\% &      80.4\% &      19.6\% &         0.004 &         -0.070 &     0.572 &    96.2\% &    84.7\% \\
       redhat &      100.0\% &      66.1\% &      33.9\% &         0.000 &         -0.226 &     0.551 &   100.0\% &   100.0\% \\
     sonatype &      100.0\% &      75.0\% &      25.0\% &         0.000 &         -0.250 &     0.667 &   100.0\% &   100.0\% \\
     \hline
         Mean &       99.5\% &      72.8\% &      27.2\% &         0.001 &         -0.204 &     0.553 &    98.3\% &    88.5\% \\
Standard Dev. &        0.9\% &       6.1\% &       6.1\% &         0.001 &          0.073 &     0.057 &     3.4\% &    12.2\% \\
% qt & 136492 & 1182 & 288 & -0.07 & 0.0 &&&&\\
% hyperledger & 27800 & 28 & 12 & -0.21 & 0.0 &&&&\\
% redhat & 315631 & 41 & 21 & -0.23 & 0.0 &&&&\\
% mongodb & 90429 & 42 & 25 & -0.32 & 0.0 &&&&\\
% mariadb & 31190 & 11 & 4 & -0.21 & 0.0 &&&&\\
% sonatype & 77825 & 3 & 1 & -0.25 & 0.0 &&&&\\
% jira & 265081 & 76 & 21 & -0.16 & 0.0 &&&&\\
% jiraecosystem & 40379 & 70 & 22 & -0.18 & 0.0 &&&&\\ % Check
\hline
    \end{tabular}
\end{table*}

==> tables/model_results_DvsOL.tex <==
\begin{table}[h!]
\setlength\tabcolsep{2.5pt}  % Adjust the table column spacing
\centering
\captionsetup{skip=0pt}
\caption{Single Channel CNN and Dual Channel CNN model results averaged over projects for the case DvsOL.}\label{tab:DvsOLResults}
\begin{tabularx}{\columnwidth}{l l L L L L} 
\hline
& \textbf{Class} & \textbf{Pre.} & \textbf{Rec.} & \textbf{F1} & \textbf{Acc.}\\
  \hline
  \multicolumn{6}{c}{On traditional \Dup{} and \NL{} test set}\\
  \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize SCCNN}}} &
 \Dup{} & 0.84 & 0.59 & 0.69 & 
 \multirow{3}{*}{0.62}\\ 
 & \NL{} & 0.41 &  0.71 & 0.49 & \\
\cline{2-5}
 & Macro avg & 0.62 & 0.65 & 0.64 & \\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize DCCNN}}} & 
 \Dup{} & 0.75 &  0.60 & 0.66 & 
 \multirow{3}{*}{0.62}  \\ 
 & \NL{} & 0.49 & 0.66 & 0.56 &  \\
\cline{2-5}
 & Macro avg & 0.62 & 0.63 & 0.62  & \\
  \hline
  
 \multicolumn{6}{c}{On test set with \OL{}}\\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize SCCNN}}} &
 \Dup{} & 0.84 (+/-0) & 0.47 (-.12) & 0.60 (-.09) & 
 \multirow{3}{*}{0.62 (+/-0)} \\ 
 & \textit{Non-Dup.}& 0.52 (+.09) &  0.47 (+.24) & 0.60 (+.11)& \\
\cline{2-5}
 & Macro avg & 0.72 (+.10) & 0.70 (+.05) & 0.71 (+.07) & \\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize DCCNN}}} & 
 \Dup{} & 0.75 (+/-0) &  0.48 (+.12) & 0.58 (+.08) & 
 \multirow{3}{*}{0.64 (+.02)}  \\ 
 & \textit{Non-Dup.}  & 0.59 (+.10) & 0.82 (+.16) & 0.68 (+.06) & \\
\cline{2-5}
 & Macro avg & 0.67 (-.05) & 0.65 (+.02) & 0.66 (+.04)  & \\
 \hline
\end{tabularx}
\end{table}

==> tables/model_results_OLMisslabels.tex <==
\begin{table}[h!]
    \small
\setlength\tabcolsep{2.5pt}  % Adjust the table column spacing
\centering
\captionsetup{skip=0pt}
\caption{Missclassification of the \OL{} as \Dup{} across projects for the DvsNL setting.}\label{tab:DvsNLResults_OL}
\begin{tabularx}{\columnwidth}{X X X} 
\hline
\textbf{Project} & \textbf{SCCNN} & \textbf{DCCNN}\\
  \hline
 Apache         & 75.8\% & 53.5\%\\
 Hyperledger    & 49.8\% & 42.1\%\\
 IntelDAOS      & 17.0\% & /\\
 JFrog          & 39.4\% & /\\
 Jira           & 84.9\% & 77.3\%\\
 JiraEcosystem  & 50.7\% & 31.9\%\\
 MariaDB        & 65.5\% & 41.8\%\\
 Mindville      & / & /\\
 MongoDB        & 72.6\% & 49.0\%\\
 Qt             & 53.2\% & 41.4\%\\
 RedHat         & 54.8\% & 34.1\%\\
 Sakai          & 48.5\% & 32.9\%\\
 Sonatype       & 67.6\% & /\\
 Spring         & 67.6\% & 38.1\%\\
 SecondLife     & / & /\\
 \hline
 \textbf{Mean} & 57.5\% & 44.2\%\\
 \textbf{Std. Var.} & 17.0\% & 13.0\%\\
\end{tabularx}
\end{table}
